Evaluating Readability and Faithfulness of Concept-based Explanations

With the growing popularity of general-purpose Large Language Models (LLMs), comes a need for more global explanations of model behaviors. Concept-based explanations arise as a promising avenue for explaining high-level patterns learned by LLMs. Yet their evaluation poses unique challenges, especially due to their non-local nature and high dimensional representation in a model's hidden space. Current methods approach concepts from different perspectives, lacking a unified formalization. This makes evaluating the core measures of concepts, namely faithfulness or readability, challenging. To bridge the gap, we introduce a formal definition of concepts generalizing to diverse concept-based explanations' settings. Based on this, we quantify the faithfulness of a concept explanation via perturbation. We ensure adequate perturbation in the high-dimensional space for different concepts via an optimization problem. Readability is approximated via an automatic and deterministic measure, quantifying the coherence of patterns that maximally activate a concept while aligning with human understanding. Finally, based on measurement theory, we apply a meta-evaluation method for evaluating these measures, generalizable to other types of explanations or tasks as well. Extensive experimental analysis has been conducted to inform the selection of explanation evaluation measures.

==> tables/faithfulness.tex <==
\begin{table*}[htbp]
    \centering
    \footnotesize
    \vspace{-20pt}
    \begin{tabular}{ccccc}
    \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Label} &  \multicolumn{3}{c}{Applicability}  \\ 
 
        \cmidrule(lr){3-5} 
        ~ & ~ & Neuron & Probing & Disentanglement \\
        
    \midrule
        Gradient-based~\cite{kim2018interpretability} & yes & \XSolidBrush & \Checkmark & \XSolidBrush  \\ 
        Disentanglement-based~\cite{schwab2019cxplain} & no & \XSolidBrush & \XSolidBrush & \Checkmark \\ 
        Probability-based~\cite{hennigen2020intrinsic} & yes & \XSolidBrush & \includegraphics[width=0.42cm]{figures/checkmarkx.png} & \XSolidBrush  \\
        GRAD/ABL (ours) & no/yes & \Checkmark & \Checkmark & \Checkmark  \\
        % ABL (ours) & no/yes & \Checkmark & \Checkmark & \Checkmark  \\
    \bottomrule
    \end{tabular}
    \vspace{-5pt}
    \caption{Comparison between mainstream faithfulness methods. }
    \label{tab:faithfulness_comparison}
    \vspace{-15pt}
\end{table*}
% \Checkmark / \XSolidBrush
